MoSSP: A Momentum-Based Single-Loop Stochastic Penalty Method for Nonconvex Constrained DC-Regularized Optimization

In this paper, we study a structured class of nonconvex constrained stochastic problems with difference-of-convex (DC) regularization, where the feasible set is possibly nonconvex and the concave part of the DC regularizer is allowed to be nonsmooth. The fundamental challenge lies in maintaining feasibility for nonconvex constraints while achieving favorable oracle complexity. Although single-loop algorithms efficiently solve unconstrained DC optimization problems, their potential for constrained optimization with DC structure remains largely unexplored. To address this gap, we develop MoSSP, a Momentum-based Single-loop Stochastic Penalty method for such problems with provable complexity guarantees. The key idea is to apply a single stochastic proximal-gradient step to the Moreau envelope of the penalty plus the convex DC part, with the concave part's proximal mapping computed in parallel. We derive two algorithm variants: a Polyak-momentum version with $O(\varepsilon^{-4})$ oracle complexity for finding stochastic $\varepsilon$-KKT points, and an improved $O(\varepsilon^{-3})$ version incorporating recursive momentum. Experimental results demonstrate the effectiveness of the proposed algorithms.

==> sections/appendices/DME_solutions_related.tex <==
\section{Appendix: Solution Correspondence for Difference-of-Moreau-Envelopes}
\label{appendix: DME properties}
In this section, we provide the complete theoretical relationship between solutions of Problem~\eqref{wcu} and its DME surrogate $\min\limits_{\bz \in \RR^n} F_\mu(\bz)$ with rigorous proofs. We first present essential mathematical tools.

\subsection{Infimal Convolution and Toland Duality}

\paragraph{\textbf{Infimal convolution \cite{moreau1971weak}.}} Let $f,\theta : \RR^n \to (-\infty,+\infty]$ be proper lower semicontinuous functions.
For any \(\bz \in \RR^n\), the infimal convolution is defined by
\begin{align}
% \label{Eq: definition infimal convolution}
(f \square \theta)(\bz) := \inf_{\bx \in \RR^n} \left\{f(\bx) + \theta(\bx - \bz)\right\}. \notag
\end{align}
When $\theta(\cdot) = \frac{1}{2\mu}\|\cdot\|^2$ for some $\mu>0$, this reduces to the \textit{Moreau envelope}:
\begin{align}
% \label{Eq: Moreau as infimal convolution}
\mathcal{M}_{\mu \phi}(\bz) = \left(\phi \square \frac{1}{2\mu}\|\cdot\|^2\right)(\bz). \notag
\end{align}
A key property \cite{borwein2006convex} states that conjugation transforms infimal convolution into summation:
\begin{align}
(f_1 \square f_2)^* = f_1^* + f_2^*, \notag
\end{align}
where, for any $\by \in \RR^n$,
\begin{align}
  f^*(\by) := \sup_{\bx \in \RR^n} \{\langle \by, \bx\rangle - f(\bx)\} \notag
\end{align}
denotes the Fenchel conjugate function of $f$.
This yields the conjugate function of the \textit{Moreau envelope}:
\begin{align}
% \label{Eq: conjugate Moreau envelope}
\mathcal{M}_{\mu \phi}^*(\by) = \phi^*(\by) + \frac{1}{2\mu}\|\by\|^2, \quad \forall\,\by \in \RR^n.\notag
\end{align}


\paragraph{\textbf{Toland duality \cite{toland1978duality}.}} The Toland dual of the objective function of Problem~\eqref{wcu} is defined as
\begin{align}
\label{Eq: Toland dual function}
F^\circ(\by) = g^*(\by) - \phi^*(\by). 
\end{align}
A key duality property of \(F\) and \(F_{\mu}\) is
\begin{align}
\label{Eq: Toland duality equality}
\inf_{\bx } F(\bx) = \inf_{\by} F^\circ(\by).
\end{align}

\subsection{Solution Correspondence Theory}
\label{App: Solution Correspondence Theory}
We now extend the solution correspondence theory of \citet{hiriart1991regularize} to the \textbf{weakly convex} setting. Let us define the optimal values $\hat{F} = \min\limits_{\bx} F(\bx)$ and $\hat{F}_{\mu} = \min\limits_{\bz} F_{\mu}(\bz)$, with the corresponding minimizer sets $\mathcal{X}_{F} = \argmin\limits_{\bx} F(\bx)$ and $\mathcal{X}_{F_{\mu}} = \argmin\limits_{\bz} F_{\mu}(\bz)$. A crucial characterization concerns the preimage of the proximal operator.
\paragraph{\textbf{Preimage characterization.}}
Let $f : \RR^n \to (-\infty,+\infty]$ be a proper lower semicontinuous function.
For any $\bx \in \RR^n$ with $\partial f(\bx) \neq \emptyset$ and any $\bxi \in \partial f(\bx)$, it holds that, for any $\mu > 0$,
\begin{align}
\label{Eq: the preimage of moreau envelope}
\mathrm{prox}_{\mu f}(\bx + \mu \bxi) = \bx.
\end{align}
This follows directly from the optimality condition of the Moreau envelope or, equivalently, from \eqref{Eq: the gradient of Moreau envelope}.

\begin{proposition}[Stationary Point and Global Minimizer Correspondence]
\label{Prop: correspondence of stationary point and global minimizer}
Consider problem \eqref{wcu}. For any $0 < \mu < \frac{1}{m_{\phi}}$, the following holds:

\textbf{(i) Stationary point correspondence.} If $\nabla F_{\mu}(\bar{\bz}) = \mathbf{0}$, then $\bar{\bx} := \textrm{prox}_{\mu\phi}(\bar{\bz})$ is a critical point of $F$ with
\begin{align}
\label{Eq: stationary identity}
\textrm{prox}_{\mu\phi}(\bar{\bz}) = \textrm{prox}_{\mu g}(\bar{\bz}), \quad F(\bar{\bx}) = F_{\mu}(\bar{\bz}).
\end{align}
Conversely, if $\bar{\bx}$ is a critical point of $F$ and $\bar{\bxi} \in \partial\phi(\bar{\bx}) \cap \partial g(\bar{\bx})$, then $\bar{\bz} = \bar{\bx} + \mu \bar{\bxi}$ is a stationary point of $F_{\mu}$ with $\textrm{prox}_{\mu \phi}(\bar{\bz}) = \textrm{prox}_{\mu g}(\bar{\bz}) = \bar{\bx}$ and $F(\bar{\bx}) = F_{\mu}(\bar{\bz})$.

\textbf{(ii) Global minimizer correspondence.}
$\mathcal{X}_{F_{\mu}} \neq \emptyset$ and $\hat{F} = \hat{F}_{\mu}$. Furthermore, if $\bar{\bz} \in \mathcal{X}_{F_{\mu}}$, then $\textrm{prox}_{\mu \phi}(\bar{\bz}) \in \mathcal{X}_{F}$; conversely, if $\bar{\bx} \in \mathcal{X}_F$ and $\bar{\bxi} \in \partial\phi(\bar{\bx}) \cap \partial g(\bar{\bx})$, then $\bar{\bz} = \bar{\bx} + \mu \bar{\bxi} \in \mathcal{X}_{F_{\mu}}$.
\end{proposition}

\begin{proof}
\textbf{Proof of Claim \textbf{(i)}.} If $\nabla F_{\mu}(\bar{\bz}) = 0$, then it holds that
\begin{align}
\mu\nabla F_{\mu}(\bar{\bz}) = \textrm{prox}_{\mu g}(\bar{\bz}) - \textrm{prox}_{\mu\phi}(\bar{\bz}) = 0, \notag
\end{align}
establishing the first equality in \eqref{Eq: stationary identity}. The function value equality in \eqref{Eq: stationary identity} follows from
\begin{align}
F(\textrm{prox}_{\mu\phi}(\bar{\bz})) 
&= \phi(\textrm{prox}_{\mu\phi}(\bar{\bz})) 
   - g(\textrm{prox}_{\mu g}(\bar{\bz})) \notag \\
&= \left[\phi(\textrm{prox}_{\mu\phi}(\bar{\bz})) 
   + \frac{1}{2\mu}\|\bar{\bz} - \textrm{prox}_{\mu\phi}(\bar{\bz})\|^2 \right]  - \left[g(\textrm{prox}_{\mu g}(\bar{\bz})) 
   + \frac{1}{2\mu}\|\bar{\bz} - \textrm{prox}_{\mu g}(\bar{\bz})\|^2 \right] \notag \\
&= \mathcal{M}_{\mu\phi}(\bar{\bz}) - \mathcal{M}_{\mu g}(\bar{\bz})
   = F_\mu(\bar{\bz}). \notag
\end{align}

For the converse, let $\bar{\bx}$ be a critical point with $\bar{\bxi} \in \partial\phi(\bar{\bx}) \cap \partial g(\bar{\bx})$ and take $\bar{\bz} = \bar{\bx} + \mu \bar{\bxi}$. By \eqref{Eq: the preimage of moreau envelope}, one has $\textrm{prox}_{\mu \phi}(\bar{\bz}) = \textrm{prox}_{\mu g}(\bar{\bz}) = \bar{\bx}$, yielding $\nabla F_{\mu}(\bar{\bz}) = 0$. The value equality follows similarly.

\textbf{Proof of Claim \textbf{(ii)}.} Since $F_{\mu}$ is $L_{F_{\mu}}$-smooth and bounded below from \Cref{Prop: smoothness of DME} (iii), it is coercive, ensuring $\mathcal{X}_{F_{\mu}} \neq \emptyset$. 
% Recalling \eqref{Eq: Toland dual function}, the Toland's dual of $F_{\mu}$ is:
% \begin{align}
% F^{\circ}_{\mu}(\bz)&= \mathcal{M}_{\mu g}(\bz) - \mathcal{M}_{\mu \phi}(\bz) \notag \\
% &= \left(g^* + \frac{1}{2\mu}\|\cdot\|^2\right) - \left(\phi^* + \frac{1}{2\mu}\|\cdot\|^2\right) \notag \\
% &= g^* - \phi^* = F^{\circ}, \notag
% \end{align}
Recalling \eqref{Eq: Toland dual function}, the Toland dual of $F_{\mu}$ is
\begin{align}
F^{\circ}_{\mu}(\by)
  &= \mathcal{M}_{\mu g}^*(\by) - \mathcal{M}_{\mu \phi}^*(\by) \notag \\
  &= \bigl(g^* + \tfrac{1}{2\mu}\|\cdot\|^2\bigr)(\by)
     - \bigl(\phi^* + \tfrac{1}{2\mu}\|\cdot\|^2\bigr)(\by) \notag \\
  &= g^*(\by) - \phi^*(\by) = F^{\circ}(\by). \notag
\end{align}
Together with \eqref{Eq: Toland duality equality}, this yields the global minimum equivalence.
% \begin{align}
% % \label{Eq: optimal value equality}
% \hat{F}_{\mu} = \inf F_{\mu} = \inf F_{\mu}^\circ = \inf F^\circ = \inf F = \hat{F}. \notag
% \end{align}


For the minimizer correspondence, it is evident that if $\bar{\bz} \in \mathcal{X}_{F_{\mu}}$, then $\bar{\bz}$ is a stationary point. From \textbf{Claim {(i)}}, $\bar{\bx} := \textrm{prox}_{\mu \phi}(\bar{\bz})$ is a critical point with
\[
F(\bar{\bx}) = F_{\mu}(\bar{\bz}) = \hat{F}_{\mu} = \hat{F},
\] yielding $\bar{\bx} \in \mathcal{X}_F$. The converse follows similarly from the second part of \textbf{Claim} \textbf{(i)}.
\end{proof}

% \begin{remark}[Key implications]
% This proposition establishes that:
% \begin{enumerate}
% \item The mapping $\textrm{prox}_{\mu\phi}$ provides a bijection between stationary points of $F_{\mu}$ and critical points of $F$;
% \item Optimal values are preserved: $\hat{F}_{\mu} = \hat{F}$;
% \item The minimizer sets correspond bijectively via $\textrm{prox}_{\mu\phi}$.
% \end{enumerate}
% These properties are fundamental for developing algorithms that solve the smooth problem $\min F_{\mu}$ to find critical points of the nonsmooth problem $\min F$.
% \end{remark}

Moreover, while \citet{sun2023algorithms} established that a local minimizer of $F$ can be obtained from a local minimizer of $F_{\mu}$ under the condition that $g$ is smooth or has bounded subgradients, the following proposition completes this result by rigorously establishing a full equivalence relationship between their local minimizers.

\begin{proposition}[Local Minimizers Correspondence]
\label{Prop: correspondence of local minimizer}
Under the conditions in \Cref{Prop: correspondence of stationary point and global minimizer}, suppose either of the following conditions on $\partial g$ holds:

\textbf{(i).} $g$ is $L_g$-smooth,

\textbf{(ii).} $\sup\limits_{\xi_g \in \partial g} \|\xi_g\| \leq M_{\partial g}$ for some \(M_{\partial g} > 0\).

Then, $\bar{\bx} := \textrm{prox}_{\mu \phi}(\bar{\bz})$ is a local minimizer of $F$ with radius $r_{\bx}> 0$ if and only if for any $\bar{\bxi} \in \partial \phi(\bar{\bx}) \cap \partial g(\bar{\bx})$, $\bar{\bz} = \bar{\bx} + \mu \bar{\bxi}$ is a local minimizer of $F_{\mu}$ with radius $r_{\bz}> 0$, where $r_{\bx}$ and $r_{\bz}$ satisfy
\begin{align}
     \label{Eq: the relationship of rx and rz}
r_x =
\begin{cases}
  \dfrac{r_z}{\mu L_g + 1}, 
    & \text{if $g$ is $L_g$-smooth,} \\[0.3ex]
  \bigl(r_z - 2\mu M_{\partial g}\bigr)\vphantom{\dfrac{r_z}{\mu L_g + 1}}, 
    & \text{if $\sup_{\xi_g \in \partial g}\|\xi_g\|\le M_{\partial g}$ and $r_z > 2\mu M_{\partial g}$.}
\end{cases}
    \end{align}
\end{proposition}

\begin{proof}
We begin with the local minimizer property of \(\bar{\bx}\). If $\bar{\bx}$ is a local minimizer of $F$ with radius \(r_{\bx}\), for any $\bar{\bxi} \in \partial \phi(\bar{\bx}) \cap \partial g(\bar{\bx})$, let us define $\bar{\bz} = \bar{\bx} + \mu \bar{\bxi}$. By \Cref{Prop: correspondence of stationary point and global minimizer}, we have $\textrm{prox}_{\mu \phi}(\bar{\bz}) = \textrm{prox}_{\mu g}(\bar{\bz}) = \bar{\bx}$.
% For any $\bx$ with $\|\bx - \bar{\bx}\| \leq r_{\bx}$ and any $\bxi \in \partial \phi(\bx) \cap \partial g(\bx)$, let us define $\bz = \bx + \mu \bxi$. Then it holds that
% \begin{align*}
% F_{\mu}(\bar{\bz}) = F(\bar{\bx}) \leq F(\bx) = F_{\mu}(\bz),
% \end{align*}
% % where the equalities follow from \Cref{Prop: correspondence of stationary point and global minimizer} and the inequality from the local minimality of $\bar{\bx}$.
% which follow from \Cref{Prop: smoothness of DME} (iii) and the properties of stationary points established in \Cref{Prop: correspondence of stationary point and global minimizer} since $\bar{\bx}$, as a local minimizer of $F$, necessarily satisfies the stationarity condition for $F$. 
For any $\bx$ with $\|\bx - \bar{\bx}\| \le r_{\bx}$ and any 
$\bxi \in \partial \phi(\bx) \cap \partial g(\bx)$, define $\bz = \bx + \mu \bxi$.
Then, one has
\begin{align*}
  F_{\mu}(\bar{\bz}) = F(\bar{\bx}) \leq F(\bx) = F_{\mu}(\bz),
\end{align*}
where the equalities follow from Proposition~\ref{Prop: correspondence of stationary point and global minimizer}
and the inequality follows from the local minimality of $\bar{\bx}$. To determine $r_{\bz}$, we bound the distance:
\begin{align*}
\|\bz - \bar{\bz}\| &= \|\bx + \mu \bxi - (\bar{\bx} + \mu \bar{\bxi})\| \leq \|\bx - \bar{\bx}\| + \mu \|\bxi - \bar{\bxi}\|.
\end{align*}

We consider the two cases separately:
\begin{itemize}
  \item[(i)] If $g$ is $L_g$-smooth, then $\|\bxi - \bar{\bxi}\| \le L_g \|\bx - \bar{\bx}\|$, yielding
  \[
    \|\bz - \bar{\bz}\| \le (1 + \mu L_g)\|\bx - \bar{\bx}\| \le (1 + \mu L_g) r_{\bx}.
  \] 
  Taking $r_{\bz} = (1 + \mu L_g) r_{\bx}$ ensures that $\|\bz - \bar{\bz}\| \le r_{\bz}$.

  \item[(ii)] If $\sup_{\xi_g \in \partial g} \|\xi_g\| \le M_{\partial g}$, then
  $\|\bxi - \bar{\bxi}\| \le 2M_{\partial g}$, yielding
  \[
    \|\bz - \bar{\bz}\| \le \|\bx - \bar{\bx}\| + 2\mu M_{\partial g}
      \le r_{\bx} + 2\mu M_{\partial g}.
  \]
Thus, by setting $r_{\bz} := r_{\bx} + 2\mu M_{\partial g}$, we obtain $\|\bz - \bar{\bz}\| \le r_{\bz}$.
\end{itemize}
In both cases, $\bar{\bz}$ is a local minimizer of $F_{\mu}$ with radius $r_{\bz}$ as in \eqref{Eq: the relationship of rx and rz}.

Conversely, if \(\bar{\bz}\) is a local minimizer of \(F_{\mu}\) with radius \(r_{\bz}\), then for any \(\bz\) satisfying \(\| \bz - \bar{\bz} \| \leq r_{\bz} \), we have
\begin{align*}
    F(\textrm{prox}_{\mu \phi}(\bar{\bz})) &= F_{\mu}(\bar{\bz})  \leq F_{\mu}(\bz) \leq F(\textrm{prox}_{\mu g}(\bz))\\
    \textrm{prox}_{\mu \phi}(\bar{\bz}) &= \textrm{prox}_{\mu g}(\bar{\bz}).
\end{align*}
Similarly, it is evident to verify that for the radius \(r_{\bx}\) satisfying \eqref{Eq: the relationship of rx and rz}, it holds that
\begin{align}
% \label{Eq: the definitin of the local minimizer of F}
F(\textrm{prox}_{\mu \phi}(\bar{\bz})) \leq F(\bx)\text{, for any \(\bx\) satisfying \(\| \bx - \textrm{prox}_{\mu \phi}(\bz)\| \leq r_{\bx}\), } \notag
\end{align}
This implies that \(\textrm{prox}_{\mu \phi}(\bar{\bz})\) is a local minimizer of \(F\) and completes the proof.
\end{proof}
\subsection{Proof of \Cref{Prop: approximate correspondence}}
\label{App: proof of prop2.2}
For the complexity analysis, we rely on the correspondence between $\varepsilon$-stationary points established in \Cref{Prop: approximate correspondence}. We provide its proof below.
\begin{proof}
We first show that an $\varepsilon$-stationary point of $F_{\mu}$ 
induces an $\varepsilon$-critical point of $F$.
Let $\bar{\bz}$ be a point satisfying $\|\nabla F_{\mu}(\bar{\bz})\|\le\varepsilon$ and set
\[
  \bar{\bx} := \mathrm{prox}_{\mu \phi}(\bar{\bz}), \qquad
  \bar{\by} := \mathrm{prox}_{\mu g}(\bar{\bz}).
\]
Using \eqref{Eq: the gradient of Moreau envelope}, we have
\[
  \bar{\bxi}_{\phi} := \mu^{-1}(\bar{\bz}-\bar{\bx}) \in \partial \phi(\bar{\bx}),
  \qquad
  \bar{\bxi}_{g} := \mu^{-1}(\bar{\bz}-\bar{\by}) \in \partial g(\bar{\by}).
\]
Combining these with \eqref{Eq: the gradient of Moreau envelope} yields
\[
  \bar{\bxi}_{\phi} - \bar{\bxi}_{g}
    = \mu^{-1}(\bar{\by}-\bar{\bx})
    = \nabla F_{\mu}(\bar{\bz}).
\]
It follows that
\begin{align*}
  \max\bigl\{\|\bar{\bxi}_{\phi}-\bar{\bxi}_{g}\|,
             \|\bar{\bx}-\bar{\by}\|\bigr\}  = \max\bigl\{\|\nabla F_{\mu}(\bar{\bz})\|,
                  \mu\|\nabla F_{\mu}(\bar{\bz})\|\bigr\} = \max\{1,\mu\}\,\|\nabla F_{\mu}(\bar{\bz})\| \leq \varepsilon.
\end{align*}
This implies that $\bar{\bx}$ is an $\varepsilon$-critical point of $F$ in the sense of Definition~\ref{Def: epsilon-critical point in DC}.

Conversely, suppose that $\bar{\bx}$ is an $\varepsilon$-critical point of $F$, so that there exist $\bar{\by}\in\RR^n$ and
$\bar{\bxi}_{\phi}\in\partial\phi(\bar{\bx})$,
$\bar{\bxi}_{g}\in\partial g(\bar{\by})$ satisfying
\[
  \max\bigl\{\|\bar{\bxi}_{\phi}-\bar{\bxi}_{g}\|,
             \|\bar{\bx}-\bar{\by}\|\bigr\} \le \varepsilon.
\]
By defining
\[
  \bar{\bz} := \bar{\bx} + \mu \bar{\bxi}_{\phi}
            =  \bar{\by} + \mu \bar{\bxi}_{g},
\] and using the preimage characterization of the proximal operator, we obtain
\[
  \mathrm{prox}_{\mu \phi}(\bar{\bz}) = \bar{\bx},
  \qquad
  \mathrm{prox}_{\mu g}(\bar{\bz}) = \bar{\by},
\]
which implies
\begin{align*} 
  \|\nabla F_{\mu}(\bar{\bz})\|
    &= \mu^{-1}\bigl\|\mathrm{prox}_{\mu g}(\bar{\bz}) 
                     - \mathrm{prox}_{\mu \phi}(\bar{\bz})\bigr\|  \\
    &= \mu^{-1}\|\bar{\by}-\bar{\bx}\|
     \leq \varepsilon.
\end{align*}
Hence $\bar{\bz}$ is an $\varepsilon$-stationary point of $F_{\mu}$, which completes the proof.
\end{proof}

